A study of X-ray flares - II. RS CVn type Binaries

We present an analysis of seven flares detected from five RS CVn-type binaries (UZ Lib, \sigma Gem, \lambda And, V711 Tau and EI Eri) observed with XMM-Newton observatory. The quiescent state X-ray luminosities in the energy band of 0.3-10.0 keV of these stars were found to be 10^{30.7-30.9} erg/s. The exponential decay time in all the sample of flares range from ~ 1 to 8 hrs. The luminosity at peak of the flares in the energy band of 0.3-10.0 keV were found to be in the range of 10^{30.8} - 10^{31.8} erg/s. The great sensitivity of the XMM-EPIC instruments allowed us to perform time resolved spectral analysis during the flares and also in the subsquent quiescent phases. The derived metal abundances of coronal plasma were found to vary during the flares observed from \sigma Gem, V771 Tau and EI Eri. In these flares elemental abundances found to be enhanced by factors of ~ 1.3-1.5 to the quiescent states. In most of the flares, the peak temperature was found to be more than 100 MK whereas emission measure increased by factors of 1.5 - 5.5. Significant sustained heating was present in the majority of flares. The loop lengths (L) derived for flaring structure were found to be of the order of 10^{10 -11} cm and are smaller than the stellar radii (R*) i.e. L/R* \lesssim 1. The flare from \sigma Gem showed a high and variable absorption column density during the flare.

==> tab_f.tex <==
\begin{deluxetable}{rcccccccc}
\tablecolumns{8}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{\leftskip0mm{Spectral parameters for each temporal segment
 of the flares as marked by vertical lines in Fig. \ref{fig:mospnlc}.\label{tab:f}}}
\setlength{\tabcolsep}{0.015in}
\tablehead{
Object (LS) & FS & $N_H$ & Z &kT& EM~&\lx & $\chi_\nu^2$ (DOF) }
\startdata
UZ Lib       (F1)& D1 & \nodata             &  \nodata                  & 4.0$_{-0.4}^{+0.5}$    & 77$_{-3}^{+3}$          & 17.98 & 0.99(315)\\
                 & D2 & \nodata             &  \nodata                  & 4.4$_{-0.5}^{+0.6}$    & 68$_{-3}^{+3}$          & 17.24 & 1.09(311)\\
                 & D3 & \nodata             &  \nodata                  & 4.9$_{-0.7}^{+0.8}$    & 57$_{-3}^{+3}$          & 16.20 & 0.97(289)\\
                 & D4 & \nodata             &  \nodata                  & 4.5$_{-0.6}^{+0.7}$    & 55$_{-3}^{+3}$          & 15.73 & 1.07(291)\\
                 & D5 & \nodata             &  \nodata                  & 3.6$_{-0.5}^{+0.6}$    & 49$_{-3}^{+3}$          & 14.28 & 1.05(283)\\
                 & D6 & \nodata             &  \nodata                  & 3.9$_{-0.6}^{+0.7}$    & 46$_{-3}^{+3}$          & 14.12 & 0.95(278)\\
                 & D7 & \nodata             &  \nodata                  & 4.6$_{-0.8}^{+1.2}$    & 35$_{-3}^{+3}$          & 13.13 & 0.91(267)\\
                 & D8 & \nodata             &  \nodata                  & 3.7$_{-0.6}^{+0.8}$    & 33$_{-3}^{+3}$          & 12.54 & 1.08(260)\\
                 & D9 & \nodata             &  \nodata                  & 3.6$_{-1.0}^{+1.7}$    & 31$_{-5}^{+6}$          & 12.29 & 1.09(89)\\
$\sigma$ Gem (F2)& R1 & 1.6$_{-0.2}^{+0.2}$ & 0.32$_{-0.02}^{+0.02}$    & 6.4$_{-0.2}^{+0.2}$    & 346$_{-6}^{+6}$         & 64.48 & 1.07(1428)\\
                 & R2 & 1.7$_{-0.2}^{+0.2}$ & 0.29$_{-0.02}^{+0.02}$    & 5.9$_{-0.2}^{+0.2}$    & 363$_{-6}^{+6}$         & 65.40 & 1.05(1345)\\
                 & R3 & 2.0$_{-0.2}^{+0.2}$ & 0.28$_{-0.02}^{+0.02}$    & 5.7$_{-0.2}^{+0.2}$    & 357$_{-7}^{+7}$         & 65.18 & 1.17(1332)\\
                 & D1 & 2.2$_{-0.2}^{+0.2}$ & 0.30$_{-0.02}^{+0.02}$    & 5.0$_{-0.1}^{+0.1}$    & 377$_{-8}^{+7}$         & 64.12 & 1.11(1367)\\
                 & D2 & 2.7$_{-0.2}^{+0.2}$ & 0.28$_{-0.02}^{+0.02}$    & 4.9$_{-0.1}^{+0.1}$    & 370$_{-8}^{+8}$         & 62.80 & 1.15(1385)\\
                 & D3 & 2.6$_{-0.2}^{+0.2}$ & 0.27$_{-0.01}^{+0.02}$    & 4.6$_{-0.1}^{+0.1}$    & 365$_{-8}^{+6}$         & 61.09 & 1.18(1361)\\
                 & D4 & 2.4$_{-0.2}^{+0.2}$ & 0.27$_{-0.02}^{+0.02}$    & 4.7$_{-0.1}^{+0.1}$    & 339$_{-7}^{+6}$         & 58.96 & 1.10(1354)\\
                 & D5 & 2.4$_{-0.2}^{+0.2}$ & 0.25$_{-0.01}^{+0.02}$    & 4.4$_{-0.1}^{+0.1}$    & 332$_{-5}^{+4}$         & 56.00 & 1.13(1308)\\
                 & D6 & 2.4$_{-0.2}^{+0.2}$ & 0.26$_{-0.02}^{+0.02}$    & 4.37$_{-0.08}^{+0.11}$ & 325$_{-5}^{+4}$         & 54.05 & 1.07(1288)\\
                 & D7 & 2.2$_{-0.2}^{+0.2}$ & 0.26$_{-0.02}^{+0.02}$    & 4.19$_{-0.08}^{+0.08}$ & 320$_{-4}^{+4}$         & 52.49 & 1.17(1263)\\
                 & D8 & 2.2$_{-0.2}^{+0.2}$ & 0.24$_{-0.02}^{+0.02}$    & 4.00$_{-0.08}^{+0.08}$ & 315$_{-5}^{+4}$         & 51.34 & 1.07(1249)\\
                 & D9 & 2.4$_{-0.2}^{+0.2}$ & 0.23$_{-0.02}^{+0.02}$    & 3.95$_{-0.08}^{+0.09}$ & 307$_{-6}^{+5}$         & 49.86 & 1.16(1223)\\
                 &D10 & 2.3$_{-0.2}^{+0.2}$ & 0.23$_{-0.02}^{+0.02}$    & 3.86$_{-0.09}^{+0.09}$ & 292$_{-5}^{+5}$         & 48.11 & 1.05(1199)\\
                 &D11 & 2.6$_{-0.2}^{+0.2}$ & 0.22$_{-0.02}^{+0.02}$    & 3.6$_{-0.08}^{+0.08}$  & 286$_{-5}^{+5}$         & 46.38 & 1.16(1166)\\
$\lambda$ And(F3)& R1 & 2.9$_{-0.7}^{+0.6}$ & 0.11$_{-0.01}^{+0.01}$    & 3.4$_{-0.4}^{+0.6}$    &  8$_{-1}^{+1}$          & 3.74  & 1.22(513)\\
                 & R2 & 3.6$_{-0.7}^{+0.6}$ & 0.09$_{-0.01}^{+0.01}$    & 4.6$_{-0.7}^{+0.8}$    &  8$_{-1}^{+1}$          & 4.15  & 1.15(551)\\
                 & R3 & 2.9$_{-0.6}^{+0.6}$ & 0.11$_{-0.01}^{+0.01}$    & 3.7$_{-0.4}^{+0.5}$    & 12$_{-1}^{+1}$          & 4.47  & 1.06(576)\\
                 & R4 & 3.2$_{-0.6}^{+0.6}$ & 0.10$_{-0.01}^{+0.01}$    & 3.8$_{-0.4}^{+0.5}$    & 12$_{-1}^{+1}$          & 4.58  & 1.13(587)\\
                 & R5 & 3.1$_{-0.7}^{+0.6}$ & 0.11$_{-0.01}^{+0.02}$    & 3.4$_{-0.4}^{+0.4}$    & 14$_{-1}^{+2}$          & 4.62  & 1.07(582)\\
                 & R6 & 2.9$_{-0.6}^{+0.6}$ & 0.11$_{-0.01}^{+0.01}$    & 2.9$_{-0.2}^{+0.2}$    & 17$_{-2}^{+2}$          & 4.61  & 1.20(587)\\
V711 Tau     (F4)& R1 & \nodata             & \nodata                   & $< 3.3$                & 2.2$_{-0.7}^{+0.7}$     & 6.1   & 0.95(511)\\
                 & D1 & \nodata             & \nodata                   & 3.9$_{-0.9}^{+1.4}$    & 6.1$_{-0.9}^{+0.9}$     & 6.5   & 1.12(523)\\
             (F5)& R1 & 1.1$_{-0.4}^{+0.6}$ & 0.205$_{-0.011}^{+0.013}$ & 2.9$_{-0.9}^{+1.3}$    &  9.5$_{-2.1}^{+3.2}$    & 7.84  & 1.32(246)\\
                 & R2 & 1.6$_{-0.5}^{+0.5}$ & 0.223$_{-0.012}^{+0.012}$ & 4.0$_{-0.5}^{+0.8}$    & 27.7$_{-2.5}^{+2.5}$    & 10.52 & 1.27(285)\\
                 & D1 & 2.0$_{-0.6}^{+0.6}$ & 0.227$_{-0.014}^{+0.021}$ & 2.6$_{-0.3}^{+0.6}$    & 36.7$_{-4.3}^{+4.3}$    & 10.75 & 1.14(250)\\
                 & D2 & 2.0$_{-0.5}^{+0.5}$ & 0.227$_{-0.013}^{+0.013}$ & 2.9$_{-0.5}^{+0.3}$    & 36.9$_{-4.6}^{+3.1}$    & 10.67 & 1.35(290)\\
                 & D3 & 2.1$_{-0.5}^{+0.5}$ & 0.234$_{-0.012}^{+0.012}$ & 2.3$_{-0.4}^{+0.3}$    & 29.5$_{-2.8}^{+4.2}$    & 9.79  & 1.10(282)\\
                 & D4 & 1.1$_{-0.4}^{+0.4}$ & 0.229$_{-0.010}^{+0.015}$ & 2.1$_{-0.2}^{+0.5}$    & 20.9$_{-3.6}^{+2.4}$    & 9.11  & 1.22(290)\\
                 & D5 & 1.6$_{-0.4}^{+0.4}$ & 0.222$_{-0.009}^{+0.009}$ & 2.0$_{-0.2}^{+0.3}$    & 16.7$_{-2.1}^{+2.1}$    & 8.39  & 1.35(315)\\
                 & D6 & 1.6$_{-0.3}^{+0.3}$ & 0.212$_{-0.008}^{+0.008}$ & 2.1$_{-0.3}^{+0.4}$    & 12.5$_{-1.8}^{+1.8}$    & 7.88  & 1.36(338)\\
             (F6)& PF & 1.1$_{-0.1}^{+0.1}$ & 0.173$_{-0.004}^{+0.003}$ & 1.8$_{-0.1}^{+0.2}$    & 11.0$_{-0.9}^{+1.0}$    & 7.29  & 1.20(627)\\
                 & R1 & 1.1$_{-0.2}^{+0.2}$ & 0.169$_{-0.005}^{+0.005}$ & 2.1$_{-0.2}^{+0.4}$    & 12.1$_{-1.7}^{+1.4}$    & 7.44  & 1.11(479)\\
                 & R2 & 1.1$_{-0.2}^{+0.2}$ & 0.170$_{-0.006}^{+0.006}$ & 2.4$_{-0.2}^{+0.2}$    & 19.2$_{-1.6}^{+1.7}$    & 8.28  & 1.10(462)\\
                 & R3 & 1.2$_{-0.2}^{+0.2}$ & 0.182$_{-0.006}^{+0.006}$ & 2.5$_{-0.2}^{+0.2}$    & 22.9$_{-1.7}^{+1.7}$    & 8.80  & 1.11(495)\\
                 & D1 & 1.3$_{-0.2}^{+0.2}$ & 0.184$_{-0.007}^{+0.004}$ & 2.4$_{-0.2}^{+0.2}$    & 25.1$_{-1.8}^{+1.8}$    & 8.96  & 1.11(527)\\
                 & D2 & 1.1$_{-0.2}^{+0.2}$ & 0.191$_{-0.006}^{+0.006}$ & 2.0$_{-0.2}^{+0.2}$    & 20.9$_{-1.7}^{+1.8}$    & 8.51  & 0.93(476)\\
                 & D3 & 0.7$_{-0.2}^{+0.2}$ & 0.188$_{-0.006}^{+0.006}$ & 2.0$_{-0.2}^{+0.3}$    & 14.7$_{-1.7}^{+1.7}$    & 8.03  & 1.13(457)\\
                 & D4 & 0.9$_{-0.2}^{+0.2}$ & 0.184$_{-0.007}^{+0.007}$ & 1.7$_{-0.3}^{+0.3}$    & 11.6$_{-1.9}^{+1.9}$    & 7.55  & 1.09(440)\\
                 & D5 & 1.1$_{-0.2}^{+0.2}$ & 0.174$_{-0.007}^{+0.007}$ & 1.6$_{-0.2}^{+0.3}$    & 11.3$_{-1.9}^{+1.9}$    & 7.28  & 1.26(430)\\
                 & D6 & 1.1$_{-0.2}^{+0.2}$ & 0.170$_{-0.005}^{+0.010}$ & 1.5$_{-0.1}^{+0.2}$    &  9.8$_{-1.7}^{+1.7}$    & 7.14  & 1.16(424)\\
                 & D7 & 1.1$_{-0.2}^{+0.2}$ & 0.165$_{-0.010}^{+0.009}$ & 1.3$_{-0.2}^{+0.2}$    & 10.4$_{-2.3}^{+2.5}$    & 7.02  & 0.96(423)\\
EI Eri       (F7)& R1 & 0.8$_{-0.4}^{+0.4}$ & 0.178$_{-0.011}^{+0.011}$ & 4.9$_{-1.1}^{+1.6}$    & 21.0$_{-2.8}^{+2.8}$    & 10.37 & 0.98(322)\\
                 & R2 & 1.3$_{-0.5}^{+0.5}$ & 0.217$_{-0.014}^{+0.014}$ & 3.7$_{-0.6}^{+0.6}$    & 45.7$_{-3.7}^{+5.6}$    & 13.64 & 1.02(319)\\
                 & D1 & $<0.8$              & 0.216$_{-0.014}^{+0.014}$ & 3.3$_{-0.5}^{+0.7}$    & 31.0$_{-4.0}^{+4.0}$    & 11.89 & 1.02(294)\\
                 & D2 & 0.5$_{-0.4}^{+0.4}$ & 0.215$_{-0.011}^{+0.011}$ & 3.2$_{-0.5}^{+0.8}$    & 16.6$_{-2.8}^{+2.8}$    & 10.09 & 0.90(323)\\
                 & D3 & 0.7$_{-0.5}^{+0.3}$ & 0.182$_{-0.010}^{+0.010}$ & 3.0$_{-0.8}^{+1.1}$    & 12.9$_{-3.6}^{+3.6}$    &  8.85 & 1.14(341)\\
                 & D4 & 0.9$_{-0.4}^{+0.4}$ & 0.174$_{-0.009}^{+0.009}$ & 3.1$_{-1.1}^{+2.5}$    &  8.2$_{-2.8}^{+2.8}$    &  8.25 & 1.12(312)\\
                 & D5 & 1.2$_{-0.4}^{+0.4}$ & 0.162$_{-0.011}^{+0.011}$ & 1.6$_{-0.4}^{+0.9}$    &  9.2$_{-3.8}^{+4.0}$    &  7.97 & 0.93(352)\\
                 & AF & 0.6$_{-0.2}^{+0.2}$ & 0.165$_{-0.005}^{+0.005}$ & 3.2$_{-0.5}^{+0.7}$    & 10.8$_{-1.4}^{+1.5}$    &  8.55 & 1.16(477)\\
\enddata
\tablenotetext{~}{{\it Note:} LS stands for light curve segments, FS stands for
``Flare Segments'', $N_H$ is in unit of $10^{20}$ cm$^{-2}$, abundances $Z$ is in solar unit, temperatures (kT) are in keV, emission measures (EM) are in $10^{52}$ cm$^{-3}$, and X-ray luminosity (\lx) is in $10^{30}$ \lum.  $\chi_\nu^2$ is the minimum reduced $\chi^2$ and DOF stands for degrees of freedom.  \tablenotetext{*}{Spectral parameters of hot component in APEC 2T fit}
}
\end{deluxetable}


